Refinement strategies for polygonal meshes applied to adaptive VEM discretization

In the discretization of differential problems on complex geometrical domains, discretization methods based on polygonal and polyhedral elements are powerful tools. Adaptive mesh refinement for such kind of problems is very useful as well and states new issues, here tackled, concerning good quality mesh elements and reliability of the simulations. In this paper we numerically investigate optimality with respect to the number of degrees of freedom of the numerical solutions obtained by the different refinement strategies proposed. A geometrically complex geophysical problem is used as test problem for several general purpose and problem dependent refinement strategies.

==> Styles/FEM.symbols.tex <==

% Questo file definisce i simboli per una serie di simboli ricorrenti
%
%
%
% Campi di numeri ed alti insiemi
%
\renewcommand{\R}{\mathop{\bf R}\nolimits}	     % Reali
%\newcommand{\Rn}{\mathop{{\bf R}^{\rm n}}\nolimits}
%\newcommand{\Rnum}[1]{\mathop{{\bf R}^{\rm #1}}\nolimits}
%\newcommand{\Rp}{\mathop{{\bf R}^{\rm +}}\nolimits}  % > 0
%\newcommand{\R}{\mathbb{R}}	     % Reali
%\newcommand{\Rn}{\mathop{{\R}^{n}}\nolimits}
\newcommand{\Rnum}[1]{\mathop{{\R}^{#1}}\nolimits}
\newcommand{\Rp}{\mathop{{\R}^{+}}\nolimits}  % > 0
\renewcommand{\N}{\mathbb{N}_+}	     % Naturali > 0
\newcommand{\Nn}{\mathop{{\N}_+^{n}}\nolimits}
\newcommand{\Nz}{\mathbb{N}}	     % Naturali + 0
\newcommand{\Nzn}{\mathop{{\Nz}^{n}}\nolimits}
\newcommand{\Z}{\mathbb{Z}}	     % interi
%
%
%
% Spazi funzionali
%
\newcommand{\leba}[1]{\mathop{{\rm L}^{#1}}\nolimits}
\newcommand{\leb}[2]{\mathop{{\rm L}^{#1}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\lebloc}[2]{\mathop{
	{\rm L}^{#1}_{\rm loc}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\lebo}[2]{\mathop{{\rm L}^{#1}_{0}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\lebdual}[2]
	{\mathop{\left({\rm L}^{#1}{\rm (}#2{\rm )}\right)'}\nolimits}
\newcommand{\sobh}[2]{\mathop{{\rm H}^{#1}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\sobho}[2]
	{\mathop{{\rm H}^{#1}_{0}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\sobhD}[2]
	{\mathop{{\rm H}^{#1}_{\rm D}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\sobhoD}[2]
	{\mathop{{\rm H}^{#1}_{\rm 0,D}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\sobhoG}[2]
	{\mathop{{\rm H}^{#1}_{\rm 0,\domG}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\sobhoDG}[2]
	{\mathop{{\rm H}^{#1}_{\rm 0,\bounddomO\bs\domG}
	{\rm (}#2{\rm )}}\nolimits}
\newcommand{\sobha}[1]{\mathop{{\rm H}^{#1}}\nolimits}
\newcommand{\sobhob}[3]
	{\mathop{{\rm H}^{#1}_{#2}{\rm (}#3{\rm )}}\nolimits}
\newcommand{\cont}[2]{\mathop{{\cal C}^{#1}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\sobhdiv}{\mathop{{\rm H}{({\rm div};}\domO{)}}\nolimits}
\newcommand{\sobhodiv}{\mathop{{\rm H_0}{({\rm div};}\domO{)}}\nolimits}
\newcommand{\W}[2]{\mathop{{\rm W}^{#1}{\rm (}#2{\rm )}}\nolimits}
\newcommand{\Wo}[2]{\mathop{{\rm W}^{#1}_{0}{\rm (}#2{\rm )}}\nolimits}
%
\newcommand{\bes}[3]{\mathop{{\rm B}^{#1}_{#2}{\rm (}#3{\rm )}}\nolimits}
\newcommand{\besa}[2]{\mathop{{\rm B}^{#1}_{#2}}\nolimits}
%
\newcommand{\Clos}[1]{\mathop{{\rm clos}_{_{#1}}}\nolimits}
\newcommand{\Span}[1]{\mathop{{\rm span}\left\{#1\right\}}\nolimits}
\newcommand{\esssup}{\mathop{{\rm ess\,sup}}\limits}
%\newcommand{\supp}{\mathop{{\rm supp}}\limits}

%
%
% Dominio
\newcommand{\domO}{{\rm \Omega}}
\newcommand{\domOC}{{\rm \overline{\Omega}}}
\newcommand{\domG}{{\rm \Gamma}}
\newcommand{\bounddomO}{{\rm \partial\domO}}
%
%
%
% \diff: Differenziale
\newcommand{\diff}{{\rm\mathstrut d}}
%
%
%
% \litin: Appartenenza senza spazi attorno
\newcommand{\litin}{\ensuremath{\!\in\!}}
%
% \lisubset: Inclusione senza spazi attorno
\newcommand{\lisubset}{\ensuremath{\!\subset\!}}
%
%
%
% Stile Matematico Calligrafico
\newcommand{\CAL}[1]{\mathop{\cal {#1}}\nolimits}
%
%
%
% Simbolo di definizione
%\newcommand{\defequal}{\stackrel{def}{=}}
\newcommand{\defequal}{=}
%
%
%%
% Vettori e Tensori
\newcommand{\VEC}[1]{\mathop{\overline{#1}}\nolimits}
%\newcommand{\TENS}[1]{\mathop{\overline{\overline{#1}}}\nolimits}
\newcommand{\TENS}[1]{\mathop{\mathbf{#1}}\nolimits}
\newcommand{\n}{\mathop{\hat{n}}\nolimits}
\newcommand{\nE}{\mathop{\hat{n}_E}\nolimits}
%
%
%
% Norme
\newcommand{\NORM}[1]{\mathop{\left\|\,#1\,\right\|}\nolimits}
\newcommand{\NORMV}[2]{\mathop{\left\|\,#1\,\right\|_{\rm #2}}\nolimits}
\newcommand{\NORMVn}[3]{\mathop{\left\|\,#1\,\right\|_{\rm #2}^{#3}}\nolimits}
\renewcommand{\norma}[1]{\mathop{\left\|\,#1\,\right\|}\nolimits}
\newcommand{\norman}[2]{\mathop{\left\|\,#1\,\right\|_{#2}}\nolimits}
\newcommand{\norm}[2]{\mathop{\left\|\,#1\,\right\|_{#2}}\nolimits}
\newcommand{\normdiv}[1]{\mathop{\left\|\,#1\,\right\|_{\rm div}}\nolimits}
\newcommand{\normn}[3]{\mathop{\left\|\,#1\,\right\|_{#2}^{#3}}\nolimits}
\newcommand{\normdivn}[2]{\mathop{\left\|\,#1\,\right\|_{\rm div}^{#2}}\nolimits}
\newcommand{\snorma}[1]{\mathop{\left|\,#1\,\right|}\nolimits}
\newcommand{\snorm}[2]{\mathop{\left|\,#1\,\right|_{#2}}\nolimits}
\newcommand{\snormn}[3]{\mathop{\left|\,#1\,\right|_{#2}^{#3}}\nolimits}
\newcommand{\enorm}[2]{\mathop{\left|\!\left|\!\left|\,#1\,\right|\!\right|\!\right|}_{#2}\nolimits}
\newcommand{\enormn}[3]{\mathop{\left|\!\left|\!\left|\,#1\,\right|\!\right|\!\right|}_{#2}^{#3}\nolimits}
%
% Prodotti Scalari
\newcommand{\DOTV}[3]{\mathop{\left(#1,#2\right)_{\rm #3}}\nolimits}
\newcommand{\DOTVn}[4]{\mathop{\left(#1,#2\right)_{\rm #3}^{#4}}\nolimits}
\newcommand{\psm}[3]{\mathop{\left(#1,#2\right)_{#3}}\nolimits}
\newcommand{\psmn}[4]{\mathop{\left(#1,#2\right)_{#3}^{#4}}\nolimits}
\newcommand{\ps}[2]{\mathop{\left(#1,#2\right)}\nolimits}
\newcommand{\psa}[3]{\mathop{\left(#1,#2\right)^{#3}}\nolimits}
%
% Dualit\`a
\newcommand{\dual}[2]{\mathop{\langle #1\,,\,#2 \rangle}\nolimits}
\newcommand{\dualm}[3]{\mathop{\langle #1\,,\,#2 \rangle_{#3}}\nolimits}
%
% Distanza
\newcommand{\dist}[2]{\mathop{d\left(#1,#2\right)}\nolimits}
%
% Traccia
\newcommand{\trace}[2]{\mathop{\gamma_{_{#1}}\!\left(#2\right)}\nolimits}
\newcommand{\invtrace}[2]{\mathop{\CAL{R}_{_{#1}}\left(#2\right)}%
								\nolimits}
%
\newcommand{\tracev}[2]{\mathop{
	\gamma^{n}_{_{#1}}\!\left(#2\right)}\nolimits}
\newcommand{\invtracev}[2]{
	\mathop{\CAL{R}^{n}_{_{#1}}\left(#2\right)}\nolimits}
%
% Spazio generico V
\newcommand{\V}{{\rm V}}
\newcommand{\Vh}{\mathop{{\rm V}_h}\nolimits}
\newcommand{\Qq}{{\rm Q}}
\newcommand{\Qqh}{\mathop{{\rm Q}_h}\nolimits}
\newcommand{\x}{{\times}}
\newcommand{\bs}{{\backslash}}
%\newcommand{\Vhl}{\mathop{\Vh^{(1)}}\nolimits}
\newcommand{\Ww}{\mathop{{\rm W}}\nolimits}
%\newcommand{\Wh}{\mathop{{\rm W}_h}\nolimits}
\newcommand{\PuT}{\mathop{\mathbb{P}_1(T)}\nolimits}
\newcommand{\PkT}{\mathop{\mathbb{P}_k(T)}\nolimits}
\newcommand{\PlT}{\mathop{\mathbb{P}_l(T)}\nolimits}
\newcommand{\PiT}{\mathop{\mathbb{P}_i(T)}\nolimits}
%
\newcommand{\PrQh}{\mathop{P_{\Qqh}}\nolimits}
\newcommand{\PrQhd}{\mathop{P_{\Qqh'}}\nolimits}
%
\newcommand{\Vu}{\mathop{{\VEC{u}}}\nolimits}
\newcommand{\Vut}{\mathop{\VEC{\tilde{u}}}\nolimits}
\newcommand{\Vv}{\mathop{{\VEC{v}}}\nolimits}
\newcommand{\IVv}{\mathop{I_h\Vv}\nolimits}
\newcommand{\VvIv}{\mathop{\Vv-I_h\Vv}\nolimits}
\newcommand{\Vf}{\mathop{{\VEC{f}}}\nolimits}
\newcommand{\VgN}{\mathop{{\VEC{g}_N}}\nolimits}
\newcommand{\Va}{\mathop{{\VEC{a}}}\nolimits}
\newcommand{\VPa}{\mathop{{\PrT\Va}}\nolimits}
\newcommand{\VPaa}{\mathop{{\PrT\Va-\Va}}\nolimits}
\newcommand{\eu}{\mathop{\VEC{\mit\Upsilon}}\nolimits}
\newcommand{\Ieu}{\mathop{I_h\eu}\nolimits}
\newcommand{\euIeu}{\mathop{\eu-I_h\eu}\nolimits}
\newcommand{\ep}{\mathop{\mit\Psi}\nolimits}
\newcommand{\VPf}{\mathop{{\PrT\Vf}}\nolimits}
\newcommand{\VPff}{\mathop{{\PrT\Vf-\Vf}}\nolimits}
\newcommand{\VPgN}{\mathop{{\PrE\VgN}}\nolimits}
\newcommand{\VPgNgN}{\mathop{{\PrE\VgN-\VgN}}\nolimits}
%
\newcommand{\Prf}{\mathop{{\PrT\!f}}\nolimits}
\newcommand{\Pfn}[1]{\mathop{{\PrT\!\fn{#1}}}\nolimits}
\newcommand{\Pffn}[1]{\mathop{{\PrT\!\fn{#1}-\fn{#1}}}\nolimits}
%
\newcommand{\Prsf}{\mathop{{\PrTs\!f}}\nolimits}
\newcommand{\Psfn}[1]{\mathop{{\PrTs\!\fn{#1}}}\nolimits}
\newcommand{\Psffn}[1]{\mathop{{\PrTs\!\fn{#1}-\fn{#1}}}\nolimits}
%
%
\newcommand{\It}{\mathop{\tilde{I}_T}\nolimits}
\newcommand{\ItVu}{\mathop{\tilde{I}_T\Vu}\nolimits}
\newcommand{\etau}{\mathop{\tilde{I}_T\Vu-\Vu}\nolimits}
\newcommand{\etap}{\mathop{\tilde{I}_T p-p}\nolimits}
\newcommand{\erruh}{\mathop{\Vu_h-\tilde{I}_T\Vu}\nolimits}
\newcommand{\errph}{\mathop{p_h-\tilde{I}_T p}\nolimits}
\newcommand{\erru}{\mathop{\Vu_h-\Vu}\nolimits}
\newcommand{\errp}{\mathop{p_h-p}\nolimits}
\newcommand{\euh}{\mathop{e_{\Vu}^h}\nolimits}
\newcommand{\eph}{\mathop{e_p^h}\nolimits}
\newcommand{\geph}{\mathop{\grad{e}_p^h}\nolimits}
\newcommand{\etu}{\mathop{\eta_{\Vu}}\nolimits}
\newcommand{\etp}{\mathop{\eta_p}\nolimits}
\newcommand{\getp}{\mathop{\grad{\eta}_p}\nolimits}
%
\newcommand{\Da}{\mathop{\left(\Va\cdot\Vnabla\right)}\nolimits}
\newcommand{\DPa}{\mathop{\left(\PrT\Va\cdot\Vnabla\right)}\nolimits}
\newcommand{\DPaa}
	{\mathop{\left(\left(\PrT\Va-\Va\right)\cdot\Vnabla\right)}\nolimits}
\newcommand{\DaPa}
	{\mathop{\left(\left(\Va-\PrT\Va\right)\cdot\Vnabla\right)}\nolimits}
%
\newcommand{\btN}{\mathop{
	\n\cdot\left(\iRe\Vnabla\Vu-p\TENS{I}\right)}\nolimits}
\newcommand{\btNh}{\mathop{
	\n\cdot\left(\iRe\Vnabla\Vu_h-p_h\TENS{I}\right)}\nolimits}
%
\newcommand{\REh}{\mathop{ \jump{
	\n_E\cdot\left(\iRe\Vnabla\Vu_h-p_h\TENS{I}\right)
				  } }\nolimits}
\newcommand{\JEh}{\mathop{\REh}\nolimits}
\newcommand{\Reh}
	{\mathop{\VEC{J}_{E}\left(\left[\Vu_h,p_h\right]\right)}\nolimits}
\newcommand{\Jeh}{\mathop{\Reh}\nolimits}
\newcommand{\Jehhat}{\mathop{\hat{\VEC{J}}_{\hat{E}}
	\left(\left[\Vu_h,p_h\right]\right)}\nolimits}
%
\newcommand{\RNh}{\mathop{\btNh-\PrE\VgN}\nolimits}
\newcommand{\Rnh}{\mathop{
	\VEC{R}_{E,N}\left(\left[\Vu_h,p_h\right],\PrE\VgN\right)
			  }\nolimits}
%
\newcommand{\RTh}{\mathop{
  -\iRe\triangle\Vu_h+\left(\PrT\Va\cdot\Vnabla\right)\Vu_h+\grad{p}_h-\PrT\Vf
			   }\nolimits}
\newcommand{\RThT}{\mathop{
  \left.-\iRe\triangle\Vu_h+\left(\PrT\Va\cdot\Vnabla\right)\Vu_h
	+\grad{p}_h-\PrT\Vf\ \right|_T
			   }\nolimits}
\newcommand{\Rth}
	{\mathop{\VEC{R}_T\left(\left[\Vu_h,p_h\right]\right)}\nolimits}
\newcommand{\Rthhat}
	{\mathop{\hat{\VEC{R}}_{\hat{T}}\left(\left[\Vu_h,p_h\right]\right)}
				\nolimits}
%
%
\newcommand{\resid}{\mathop{\Theta_{R_{T,E,N}}}\nolimits}
\newcommand{\residq}{\mathop{\Theta_{R_{T,E,N}}^2}\nolimits}
\newcommand{\data}{\mathop{\Lambda_{data}}\nolimits}
\newcommand{\datat}{\mathop{\tilde{\Lambda}_{data}}\nolimits}
%
%
\newcommand{\wT}{\mathop{\VEC{w}_T}\nolimits}
\newcommand{\wThat}{\mathop{\hat{\VEC{w}}_{\hat{T}}}\nolimits}
\newcommand{\wt}{\mathop{w_T}\nolimits}
\newcommand{\divwT}{\mathop{\VEC{\nabla}\cdot\wT}\nolimits}
\newcommand{\wE}{\mathop{\VEC{w}_E}\nolimits}
\newcommand{\wEhat}{\mathop{\hat{\VEC{w}}_{\hat{E}}}\nolimits}
\newcommand{\wEBz}{\mathop{\VEC{w}_{E,\Btheta}}\nolimits}
\newcommand{\wEhatBz}{\mathop{\hat{\VEC{w}}_{\hat{E},\Btheta}}\nolimits}
\newcommand{\divwE}{\mathop{\VEC{\nabla}\cdot\wE}\nolimits}
\newcommand{\divwEBz}{\mathop{\VEC{\nabla}\cdot\wEBz}\nolimits}
%
\newcommand{\vIv}{\mathop{\Vv-I_h\Vv}\nolimits}
%
%
%
% Operatori differenziali
%\newcommand{\grad}[1]{\mathop{\VEC{\nabla #1}}\nolimits}
\newcommand{\dive}[1]{\mathop{\VEC{\nabla}\cdot\VEC{#1}}\nolimits}
\newcommand{\divp}[1]{\mathop{\VEC{\nabla}\cdot\left(#1\right)}\nolimits}
\newcommand{\nd}{\mathop{\Vnabla\cdot}\nolimits}
\newcommand{\Vnabla}{\mathop{\VEC{\nabla}}\nolimits}
\newcommand{\ddn}[1]{\mathop{\ds\frac{\partial #1}{\partial\hat{n}}}\nolimits}
\newcommand{\Imm}{\mathop{{\rm Im}}\nolimits}
\newcommand{\Ker}{\mathop{{\rm Ker}}\nolimits}
%
\newcommand{\BB}{{Babu\v{s}ka-Brezzi}}
%
%
%
%
% Decomposizione del dominio ecc.
%\newcommand{\T}{\mathop{{\cal T}}\nolimits}
\newcommand{\Th}{\mathop{{\cal T}_h}\nolimits}
\newcommand{\Thr}{\mathop{{\cal T}_{h_r}}\nolimits}
\newcommand{\To}{\mathop{\stackrel{\circ}{T}}\nolimits}
\newcommand{\upt}{\mathop{\sharp}\nolimits}
\newcommand{\downt}{\mathop{\flat}\nolimits}
%\newcommand{\Tu}{\mathop{T_{\upt}}\nolimits}
%\newcommand{\Td}{\mathop{T_{\downt}}\nolimits}
\newcommand{\nTu}{\mathop{\hat{n}_{\upt}}\nolimits}
\newcommand{\nTd}{\mathop{\hat{n}_{\downt}}\nolimits}
\newcommand{\gTu}{\mathop{\grad{\varphi}_{\upt}}\nolimits}
\newcommand{\gTd}{\mathop{\grad{\varphi}_{\downt}}\nolimits}
%
%
%
% Numero di nodi, elementi,...
\newcommand{\Nnode}{\mathop{N_{node}}\nolimits}
\newcommand{\Nele}{\mathop{N_{ele}}\nolimits}
%
% Elemento finito triangolare
%
\newcommand{\Dx}[1]{\mathop{\delta_{x_{#1}}}\nolimits}
\newcommand{\Dy}[1]{\mathop{\delta_{y_{#1}}}\nolimits}
%
%
%
% h MINIMO e h MASSIMO
\newcommand{\hmin}{\mathop{\check{h}}}
\newcommand{\hmax}{\mathop{h}}
%
%
%
% Costante C in tondo normale per tutte le occasioni
%
\newcommand{\Cst}{{\rm C}}
\newcommand{\TOL}{{\rm TOL}}
\newcommand{\TOLO}{{\rm TOL}_{\Omega}}
\newcommand{\TOLt}{{\rm TOL}_{\InC}}
\newcommand{\CP}{\mathop{C_{\domO}}\nolimits}
\newcommand{\CPq}{\mathop{C_{\domO}^2}\nolimits}
\newcommand{\iCP}{\mathop{\frac{1}{\CP}}\nolimits}
\newcommand{\iCPq}{\mathop{\frac{1}{\CPq}}\nolimits}
\newcommand{\CG}{\mathop{C_{\domG}}\nolimits}
\newcommand{\CGs}{\mathop{C_{\domG}^*}\nolimits}
\newcommand{\CGN}{\mathop{C_{\domG_N}}\nolimits}
\newcommand{\CGNq}{\mathop{C_{\domG_N}^2}\nolimits}
\newcommand{\iCGN}{\mathop{\frac{1}{\CGN}}\nolimits}
\newcommand{\iCGNq}{\mathop{\frac{1}{\CGNq}}\nolimits}
\newcommand{\CPGN}{\mathop{C_{\domO,\domG_N}}\nolimits}
\newcommand{\CuGN}{\mathop{C_{1,\domG_N}}\nolimits}
\newcommand{\iCuGN}{\mathop{\frac{1}{\CuGN}}\nolimits}
\newcommand{\kc}{\mathop{\alpha}\nolimits}
\newcommand{\kBB}{\mathop{\beta}\nolimits}
\newcommand{\kBBz}{\mathop{\beta}\nolimits}
\newcommand{\cinf}{\mathop{\underline{c}}\nolimits}
\newcommand{\csup}{\mathop{\overline{C}}\nolimits}
\newcommand{\calcinf}{\mathop{\underline{\CAL{C}}}\nolimits}
\newcommand{\calcsup}{\mathop{\overline{\CAL{C}}}\nolimits}
\newcommand{\oot}{\mathop{\frac{1}{2}}\nolimits}
%
%
%
% numero di Reynolds e Bz
%
\newcommand{\iRe}{\mathop{\frac{1}{Re}}\nolimits}
\newcommand{\isqRe}{\mathop{\frac{1}{\sqrt{Re}}}\nolimits}
\newcommand{\isqfRe}{\mathop{\frac{1}{\sqrt[4]{Re}}}\nolimits}
\newcommand{\Bz}{\mathop{z}\nolimits}
\newcommand{\iBz}{\mathop{\frac{1}{\Bz}}\nolimits}
\newcommand{\isqBz}{\mathop{\frac{1}{\sqrt{\Bz}}}\nolimits}
%
%
%
%
% Misure e Proiettori
\newcommand{\mis}[1]{\mathop{\ds\left|\,#1\,\right|}\nolimits}
\newcommand{\PrT}{\mathop{\Pi_T}\nolimits}
\newcommand{\PrE}{\mathop{\Pi_E}\nolimits}
%
\newcommand{\PrTs}{\mathop{\Pi_{\Ts}}\nolimits}
\newcommand{\PrEs}{\mathop{\Pi_{\Es}}\nolimits}
%
%
%
%
% Insiemi dei lati della triangolazione
\newcommand{\ET}{\mathop{\CAL{E}(T)}\nolimits}
\newcommand{\ETs}{\mathop{\CAL{E}(\Ts)}\nolimits}
\newcommand{\ETp}{\mathop{\CAL{E}(\Tp)}\nolimits}
\newcommand{\EH}{\mathop{\CAL{E}_{h}}\nolimits}
\newcommand{\EO}{\mathop{\CAL{E}_{h,\domO}}\nolimits}
\newcommand{\ED}{\mathop{\CAL{E}_{h,D}}\nolimits}
\newcommand{\EN}{\mathop{\CAL{E}_{h,N}}\nolimits}
\newcommand{\Eh}[1]{\mathop{\CAL{E}_{h,#1}}\nolimits}
%
%
%
%
% Insiemi di triangoli
\newcommand{\oT}{\mathop{\omega_T}\nolimits}
\newcommand{\oTt}{\mathop{\tilde{\omega}_T}\nolimits}
\newcommand{\oE}{\mathop{\omega_E}\nolimits}
\newcommand{\oEt}{\mathop{\tilde{\omega}_E}\nolimits}
\newcommand{\ox}{\mathop{\omega_x}\nolimits}
\newcommand{\boundT}{\mathop{\partial T}\nolimits}
\newcommand{\boundTp}{\mathop{\partial \Tp}\nolimits}
%
%
%
% Residuo e Salti
%\newcommand{\RE}[1]{\mathop{R_E\left(#1\right)}\nolimits}
%\newcommand{\jump}[1]
%	{\mathop{ \left[#1\right]_{\bf E} }\nolimits}
%\newcommand{\jump}[1]
%	{\mathop{ \left[#1\right]_{E} }\nolimits}
\newcommand{\jump}[1]
	{\mathop{ \left[\!\!\left[#1\right]\!\!\right]_{E} }\nolimits}
\newcommand{\jumpS}[1]
	{\mathop{ \left[\!\!\left[#1\right]\!\!\right]_{S} }\nolimits}
\newcommand{\jumpSm}[1]
	{\mathop{ \left[\!\!\left[#1\right]\!\!\right]_{S_m} }\nolimits}
\newcommand{\jumpSd}[1]
	{\mathop{ \left[\!\!\left[#1\right]\!\!\right]_{S_2} }\nolimits}
% \newcommand{\jumps}[1]
% 	{\mathop{ \left[\!\!\left[#1\right]\!\!\right]_{\Es} }\nolimits}
%
%
%
% Indicatore d'errore
\newcommand{\alfam}{\mathop{(1-\alpha)}\nolimits}
\newcommand{\alfap}{\mathop{(1+\alpha)}\nolimits}
\newcommand{\alfainf}{\mathop{\alpha_{inf}}\nolimits}
\newcommand{\alfasup}{\mathop{\alpha_{sup}}\nolimits}
\newcommand{\UCDalfam}{\mathop{(1-\alfainf)}\nolimits}
\newcommand{\UCDalfap}{\mathop{(1+\alfasup)}\nolimits}
\newcommand{\etaRT}{\mathop{\eta_{R,T}}\nolimits}
\newcommand{\etaRTq}{\mathop{\eta_{R,T}^2}\nolimits}
\newcommand{\etaO}{\mathop{\eta_{_{\Omega}}}\nolimits}
\newcommand{\etaOq}{\mathop{\eta^2_{_{\Omega}}}\nolimits}
\newcommand{\etaRTmid}{\mathop{\overline{\eta^2}_{R,T}}\nolimits}
\newcommand{\etaRTqMAX}{\mathop{\eta^2_{R,T,MAX}}\nolimits}
\newcommand{\etaRTqmin}{\mathop{\eta^2_{R,T,min}}\nolimits}
%\newcommand{\etaRTqrms}{\mathop{\eta^2_{R,T,rms}}\nolimits}
\newcommand{\etaRTqrms}{\mathop{\sigma_{\etaRTq}}\nolimits}
\newcommand{\teAlphaQ}{\mathop{\AlphaQ\enorm{\eu}{\domO}
				+\norm{\ep}{0}}\nolimits}
\newcommand{\te}{\mathop{\snorm{\eu}{1}+\norm{\ep}{0}}\nolimits}
\newcommand{\tezLp}{\mathop{\normdiv{\eu}+\norm{\ep}{0}}\nolimits}
\newcommand{\tezLpSF}{\mathop{\normdiv{\eu}+\norm{\grad{\ep}}{0}}\nolimits}
\newcommand{\normref}{\mathop{\snorm{\Vu_h}{1}+\norm{p_h}{0}}\nolimits}
\newcommand{\tre}{\mathop{\frac{\te}{\normref}}\nolimits}
%
%
%
% Navier-Stokes
\newcommand{\up}{\mathop{[\Vu,p]}\nolimits}
\newcommand{\vq}{\mathop{[\Vv,q]}\nolimits}
%
%
%
% Problema test
\newcommand{\eRx}{\mathop{{e^{{R_1}x}}}\nolimits}
\newcommand{\eRu}{\mathop{{e^{{R_1}}}}\nolimits}
\newcommand{\eRxq}{\mathop{{e^{2{R_1}x}}}\nolimits}
\newcommand{\cosRx}{\mathop{
	\cos\left(
	{\frac{2\,\pi\,\left(\eRx-1\right)}{\eRu-1}}
						\right)}\nolimits}

\newcommand{\sinRx}{\mathop{
	\sin\left(
	{\frac{2\,\pi\,\left(\eRx-1\right)}{\eRu-1}}
						\right)}\nolimits}
%
\newcommand{\eRy}{\mathop{{e^{{R_2}y}}}\nolimits}
\newcommand{\eRd}{\mathop{{e^{{R_2}}}}\nolimits}
\newcommand{\eRyq}{\mathop{{e^{2{R_2}y}}}\nolimits}
\newcommand{\cosRy}{\mathop{
	\cos\left(
	{\frac{2\,\pi\,\left(\eRy-1\right)}{\eRd-1}}
						\right)}\nolimits}

\newcommand{\sinRy}{\mathop{
	\sin\left(
	{\frac{2\,\pi\,\left(\eRy-1\right)}{\eRd-1}}
						\right)}\nolimits}
%
%
%
% Zero order term
\newcommand{\RThz}{\mathop{
  -\iRe\triangle\Vu_h+\DPa\Vu_h+\Bz \Vu_h+\Vnabla p_h-\VPf
			   }\nolimits}
\newcommand{\RThzLp}{\mathop{\Vu_h+\Vnabla p_h-\VPf}\nolimits}
\newcommand{\Rthz}
	{\mathop{\VEC{R}_T\left(\left[\Vu_h,p_h\right]\right)}\nolimits}
\newcommand{\RthzLp}
	{\mathop{\VEC{R}_T\left(\left[\Vu_h,p_h\right]\right)}\nolimits}
% costanti \alpha varie
%
\newcommand{\Alpha}[1]{\mathop{\alpha_{1,#1}}\nolimits}
\newcommand{\AlphaG}{\mathop{\alpha_1}\nolimits}
\newcommand{\AlphaD}{\mathop{\alpha_2}\nolimits}
\newcommand{\AlphaT}{\mathop{\alpha_3}\nolimits}
\newcommand{\AlphaQ}{\mathop{\alpha_4}\nolimits}
\newcommand{\AlphaC}[1]{\mathop{\alpha_{5,#1}}\nolimits}
\newcommand{\AlphaCG}{\mathop{\alpha_5}\nolimits}
\newcommand{\AlphaS}[1]{\mathop{\alpha_{6,#1}}\nolimits}
\newcommand{\AlphaSG}{\mathop{\alpha_6}\nolimits}
\newcommand{\AlphaSGbar}{\mathop{\bar{\alpha}_6}\nolimits}
\newcommand{\AlphaST}[1]{\mathop{\alpha_{7,#1}}\nolimits}
\newcommand{\AlphaSTG}{\mathop{\alpha_7}\nolimits}
\newcommand{\AlphaSTGbar}{\mathop{\bar{\alpha}_7}\nolimits}
%
\newcommand{\Alphaq}[1]{\mathop{\alpha_{1,#1}^2}\nolimits}
\newcommand{\AlphaGq}{\mathop{\alpha_1^2}\nolimits}
\newcommand{\AlphaDq}{\mathop{\alpha_2^2}\nolimits}
\newcommand{\AlphaTq}{\mathop{\alpha_3^2}\nolimits}
\newcommand{\AlphaTqq}{\mathop{\alpha_3^4}\nolimits}
\newcommand{\AlphaQq}{\mathop{\alpha_4^2}\nolimits}
\newcommand{\AlphaCq}[1]{\mathop{\alpha_{5,#1}^2}\nolimits}
\newcommand{\AlphaCGq}{\mathop{\alpha_5^2}\nolimits}
\newcommand{\AlphaSq}[1]{\mathop{\alpha_{6,#1}^2}\nolimits}
\newcommand{\AlphaSGq}{\mathop{\alpha_6^2}\nolimits}
\newcommand{\AlphaSGbarq}{\mathop{\bar{\alpha}_6^2}\nolimits}
\newcommand{\AlphaSTq}[1]{\mathop{\alpha_{7,#1}^2}\nolimits}
\newcommand{\AlphaSTGq}{\mathop{\alpha_7^2}\nolimits}
\newcommand{\AlphaSTGbarq}{\mathop{\bar{\alpha}_7^2}\nolimits}
%
\newcommand{\Btheta}{\mathop{\theta}\nolimits}
\newcommand{\isqBtheta}{\mathop{\frac{1}{sqrt{\Btheta}}}\nolimits}
\newcommand{\BTheta}[1]{\mathop{\Btheta_{#1}}\nolimits}
\newcommand{\isqBTheta}[1]{\mathop{\frac{1}{\sqrt{\Btheta_{#1}}}}\nolimits}
%
\newcommand{\BetaU}[1]{\mathop{\beta_{1,E,#1,\Btheta_{#1}}}\nolimits}
\newcommand{\BetaC}[1]{\mathop{\beta_{5,E,#1,\Btheta_{#1}}}\nolimits}
\newcommand{\BetaCq}[1]{\mathop{\beta_{5,E,#1,\Btheta_{#1}}^2}\nolimits}
%
\newcommand{\GammaUT}[1]{\mathop{\gamma_{1,E,#1,\Btheta_{#1}}}\nolimits}
\newcommand{\GammaU}[1]{\mathop{\gamma_{1,E,#1}}\nolimits}
\newcommand{\GammaUtot}[1]{\mathop{\gamma_{1,#1}}\nolimits}
\newcommand{\GammaCT}[1]{\mathop{\gamma_{5,E,#1,\Btheta_{#1}}}\nolimits}
\newcommand{\GammaCTq}[1]{\mathop{\gamma_{5,E,#1,\Btheta_{#1}}^2}\nolimits}
%
\newcommand{\RhoC}[1]{\mathop{\rho_{5,#1}}\nolimits}
\newcommand{\RhoCq}[1]{\mathop{\rho_{5,#1}^2}\nolimits}
%
\newcommand{\AlphaStheta}[1]{\mathop{\alpha_{6,#1,\Btheta_{#1}}}\nolimits}
\newcommand{\AlphaSqtheta}[1]{\mathop{\alpha_{6,#1,\Btheta_{#1}}^2}\nolimits}
\newcommand{\AlphaSTtheta}[1]{\mathop{\alpha_{7,#1,\Btheta_{#1}}}\nolimits}
\newcommand{\AlphaSTqtheta}[1]{\mathop{\alpha_{7,#1,\Btheta_{#1}}^2}\nolimits}
%
\newcommand{\AlphaSGtheta}{\mathop{\alpha_{6,\Btheta}}\nolimits}
\newcommand{\AlphaSqGtheta}{\mathop{\alpha_{6,\Btheta}^2}\nolimits}
\newcommand{\AlphaSTGtheta}{\mathop{\alpha_{7,\Btheta}}\nolimits}
\newcommand{\AlphaSTqGtheta}{\mathop{\alpha_{7,\Btheta}^2}\nolimits}
%
% Convection Diffusion
\newcommand{\tI}{\mathop{(0,\Xi)}\nolimits}
\newcommand{\tn}[1]{\mathop{t^{#1}}\nolimits}
\newcommand{\tIn}{\mathop{\left(\tn{n-1},\tn{n}\right)}\nolimits}
\newcommand{\tInC}{\mathop{\left[\tn{n-1},\tn{n}\right]}\nolimits}
\newcommand{\InC}{\mathop{I^{n}}\nolimits}
\newcommand{\Dtn}{\mathop{\Delta\!\tn{n}}\nolimits}
\newcommand{\Dt}{\mathop{\Delta\!t}\nolimits}
%
\newcommand{\dudt}{\mathop{\frac{\partial u}{\partial t}}\nolimits}
\newcommand{\un}[1]{\mathop{u^{#1}}\nolimits}
\newcommand{\unh}[1]{\mathop{u^{#1}_{h,\Dt}}\nolimits}
\newcommand{\vnh}[1]{\mathop{v^{#1}_{h,\Dt}}\nolimits}
\newcommand{\uS}{\mathop{u^{n}_{h,\Dt}}\nolimits}
\newcommand{\uSc}{\mathop{u_{h,\Dt}}\nolimits}
\newcommand{\duSdt}{\mathop{\frac{\partial\uS}{\partial t}}\nolimits}
\newcommand{\duScdt}{\mathop{\frac{\partial\uSc}{\partial t}}\nolimits}
%\newcommand{\utnh}[1]{\mathop{u^{#1}_{h,\Dt}}\nolimits}
\newcommand{\usdn}[1]{\mathop{u^{#1}_{\Dt}}\nolimits}
%
%\newcommand{\Projhkn}{\mathop{P^{n}_{1;h,k}}\nolimits}
%\newcommand{\Phkn}[1]{\mathop{P^{n}_{1;h,k} #1}\nolimits}
%\newcommand{\Projhko}{\mathop{P^{[0]}_{1;h,k}}\nolimits}
%\newcommand{\Phko}[1]{\mathop{P^{[0]}_{1;h,k} #1}\nolimits}
\newcommand{\Projhkn}{\mathop{P^{n}_{h,k}}\nolimits}
\newcommand{\Phkn}[1]{\mathop{P^{n}_{h,k} #1}\nolimits}
\newcommand{\Projhko}{\mathop{P^{1}_{h,k}}\nolimits}
\newcommand{\Phko}[1]{\mathop{P^{1}_{h,k} #1}\nolimits}
%
\newcommand{\inthkn}{\mathop{{\pi}^{n}_{h,k}}\nolimits}
\newcommand{\pinthkn}[1]{\mathop{{\pi}^{n}_{h,k}\left(#1\right)}\nolimits}
\newcommand{\inthko}{\mathop{{\pi}^{1}_{h,k}}\nolimits}
\newcommand{\pinthko}[1]{\mathop{{\pi}^{1}_{h,k}\left(#1\right)}\nolimits}
%
\newcommand{\Vanh}[1]{\mathop{\Va^{#1}}\nolimits}
\newcommand{\Dau}{\mathop{\Va\cdot\nabla u}\nolimits}
\newcommand{\Dav}{\mathop{\Va\cdot\nabla v}\nolimits}
\newcommand{\Daun}[1]{\mathop{\Va^{#1}\cdot\nabla\un{#1}}\nolimits}
\newcommand{\Daunh}[2]{\mathop{\Va^{#1}\cdot\nabla\unh{#2}}\nolimits}
%\newcommand{\Dautnh}[1]{\mathop{\Va^{#1}\cdot\nabla\utnh{#1}}\nolimits}
\newcommand{\DauS}{\mathop{\Va\cdot\nabla\uS}\nolimits}
\newcommand{\Davnh}[1]{\mathop{\Va^{#1}\cdot\nabla v_h}\nolimits}
%
\newcommand{\fn}[1]{\mathop{f^{#1}}\nolimits}
%
\newcommand{\lebOT}[2]{\mathop{{\rm L}^{#1}{\rm (}\left(0,\Xi\right);#2{\rm)}}\nolimits}
%\newcommand{\lebt}[2]{\mathop{{\rm L}^{#1}{\rm (}\left(\tn{n-1},\tn{n}\right);#2{\rm )}}\nolimits}
\newcommand{\lebt}[2]{\mathop{{\rm L}^{#1}{\rm (}\InC;#2{\rm )}}\nolimits}
\newcommand{\lebtInC}[2]{\mathop{{\rm L}^{#1}{\rm (}\tInC;#2{\rm )}}\nolimits}
\newcommand{\dualnm}[2]{\mathop{\left\langle #1,#2 \right\rangle}\nolimits}
\newcommand{\contOT}[2]{\mathop{{\cal C}^{#1}{\rm (}[0,\Xi];#2{\rm )}}\nolimits}
\newcommand{\contn}[2]{\mathop{{\cal C}^{#1}{\rm (}[\tn{n-1},\tn{n}];#2{\rm )}}\nolimits}
\newcommand{\contIn}[2]{\mathop{{\cal C}^{#1}{\rm (}\InC;#2{\rm )}}\nolimits}
%
\newcommand{\iPe}{\mathop{\frac{1}{Pe}}\nolimits}
\newcommand{\iPeq}{\mathop{\frac{1}{Pe^2}}\nolimits}
\newcommand{\isqPe}{\mathop{\frac{1}{\sqrt{Pe}}}\nolimits}
%
%
\newcommand{\kk}{\mathop{\kappa}\nolimits}
\newcommand{\kkx}{\mathop{\kappa(x)}\nolimits}
\newcommand{\ikk}{\mathop{\frac{1}{\kk}}\nolimits}
\newcommand{\ikkx}{\mathop{\frac{1}{\kkx}}\nolimits}
\newcommand{\sqkk}{\mathop{\sqrt{\kk}}\nolimits}
\newcommand{\sqkkx}{\mathop{\sqrt{\kkx}}\nolimits}
\newcommand{\isqkk}{\mathop{\frac{1}{\sqrt{\kk}}}\nolimits}
%
\newcommand{\kkT}{\mathop{\kappa_T}\nolimits}
\newcommand{\ikkT}{\mathop{\frac{1}{\kkT}}\nolimits}
\newcommand{\sqkkT}{\mathop{\sqrt{\kkT}}\nolimits}
\newcommand{\isqkkT}{\mathop{\frac{1}{\sqrt{\kkT}}}\nolimits}
%
\newcommand{\kkTs}{\mathop{\kappa_{\Ts}}\nolimits}
\newcommand{\ikkTs}{\mathop{\frac{1}{\kkTs}}\nolimits}
\newcommand{\sqkkTs}{\mathop{\sqrt{\kkTs}}\nolimits}
\newcommand{\isqkkTs}{\mathop{\frac{1}{\sqrt{\kkTs}}}\nolimits}
%
\newcommand{\kkTp}{\mathop{\kappa_{\Tp}}\nolimits}
\newcommand{\ikkTp}{\mathop{\frac{1}{\kkTp}}\nolimits}
\newcommand{\sqkkTp}{\mathop{\sqrt{\kkTp}}\nolimits}
\newcommand{\isqkkTp}{\mathop{\frac{1}{\sqrt{\kkTp}}}\nolimits}
%
\newcommand{\kkE}{\mathop{\hat{\kappa}_{\oEn}}\nolimits}
\newcommand{\kkEx}{\mathop{\hat{\kappa}_{\oEn}(x)}\nolimits}
\newcommand{\ikkE}{\mathop{\frac{1}{\kkE}}\nolimits}
\newcommand{\sqkkE}{\mathop{\sqrt{\kkE}}\nolimits}
\newcommand{\sqkkEx}{\mathop{\sqrt{\kkEx}}\nolimits}
\newcommand{\isqkkE}{\mathop{\frac{1}{\sqrt{\kkE}}}\nolimits}
\newcommand{\isqkkEx}{\mathop{\frac{1}{\sqrt{\kkEx}}}\nolimits}
%
\newcommand{\kkEs}{\mathop{\hat{\kappa}_{\oEsn}}\nolimits}
\newcommand{\ikkEs}{\mathop{\frac{1}{\kkEs}}\nolimits}
\newcommand{\sqkkEs}{\mathop{\sqrt{\kkEs}}\nolimits}
\newcommand{\isqkkEs}{\mathop{\frac{1}{\sqrt{\kkEs}}}\nolimits}
\newcommand{\kkEsx}{\mathop{\hat{\kappa}_{\oEsn}(x)}\nolimits}
\newcommand{\sqkkEsx}{\mathop{\sqrt{\kkEsx}}\nolimits}
\newcommand{\isqkkEsx}{\mathop{\frac{1}{\sqrt{\kkEsx}}}\nolimits}
%
\newcommand{\ikkEd}{\mathop{\frac{1}{\kkEd}}\nolimits}
\newcommand{\sqkkEd}{\mathop{\sqrt{\kkEd}}\nolimits}
\newcommand{\isqkkEd}{\mathop{\frac{1}{\sqrt{\kkEd}}}\nolimits}
%
\newcommand{\kkoT}{\mathop{\hat{\kappa}_{\oTtn}}\nolimits}
\newcommand{\ikkoT}{\mathop{\frac{1}{\kkoT}}\nolimits}
\newcommand{\sqkkoT}{\mathop{\sqrt{\kkoT}}\nolimits}
\newcommand{\isqkkoT}{\mathop{\frac{1}{\sqrt{\kkoT}}}\nolimits}
%
\newcommand{\LT}{\mathop{\Lambda_{\oTtn}}\nolimits}
\newcommand{\LE}{\mathop{\Lambda_{\oEtn}}\nolimits}
%
\newcommand{\Thn}[1]{\mathop{{\cal T}_h^{#1}}\nolimits}
\newcommand{\Thdn}[2]{\mathop{{\cal T}_{h,{#1}}^{#2}}\nolimits}
%\newcommand{\ThnE}[1]{\mathop{{\cal
%	T}_{h^{[n-1,n]},\stackrel{_\diamond}{\omega}^{[n-1,n]}}}\nolimits}
\newcommand{\ThnE}{\mathop{{\cal T}^{n-1,n}_{h,\stackrel{_\diamond}{\omega}}}\nolimits}
%\newcommand{\Thntr}[1]{\mathop{{\cal T}_{h,J_{tr}}^{#1}}\nolimits}
\newcommand{\Thntr}[1]{\mathop{{\cal T}_{h,tr}^{#1}}\nolimits}
\newcommand{\hTn}[1]{\mathop{h_T^{#1}}\nolimits}
\newcommand{\hEn}[1]{\mathop{h_E^{#1}}\nolimits}
\newcommand{\hTsn}[1]{\mathop{h_{\Ts}^{#1}}\nolimits}
\newcommand{\hEsn}[1]{\mathop{h_{\Es}^{#1}}\nolimits}
\newcommand{\hTpn}[1]{\mathop{h_{\Tp}^{#1}}\nolimits}
\newcommand{\hn}[1]{\mathop{h^{#1}}\nolimits}
\newcommand{\hminn}[1]{\mathop{h_{min}^{#1}}\nolimits}
\newcommand{\Vhn}[1]{\mathop{{\rm V}_h^{#1}}\nolimits}
%
\newcommand{\xhn}{\mathop{x_h^{n}}\nolimits}
\newcommand{\xhnn}[1]{\mathop{x_h^{#1}}\nolimits}
\newcommand{\xhni}{\mathop{x_{h,i}^{n}}\nolimits}
%\newcommand{\Nhn}[1]{\mathop{{\cal{N}}_h^{n}\left(#1\right)}\nolimits}
%\newcommand{\Nhnn}[2]{\mathop{{\cal{N}}_h^{#2}\left(#1\right)}\nolimits}
\newcommand{\Nhn}{\mathop{{\cal{N}}_h^{n}}\nolimits}
\newcommand{\Nhntr}{\mathop{{\cal{N}}_{h,tr}^{n}}\nolimits}
\newcommand{\Nhnpr}{\mathop{{\cal{N}}_{h,p_r}^{n}}\nolimits}
\newcommand{\Nhnn}[1]{\mathop{{\cal{N}}_h^{#1}}\nolimits}
\newcommand{\Nhdn}[2]{\mathop{{\cal{N}}_{h,#1}^{#2}}\nolimits}
\newcommand{\Tmax}{\mathop{\hat{T}_{\xhn}}\nolimits}
\newcommand{\Tmaxi}{\mathop{\hat{T}_{\xhni}}\nolimits}
\newcommand{\oxn}{\mathop{\omega_{\xhn}}\nolimits}
\newcommand{\oxTn}{\mathop{\tilde{\omega}_{T,\xhn}}\nolimits}
\newcommand{\oxTnn}{\mathop{\tilde{\omega}_{T,\xhnn{n-1,n}}}\nolimits}
%
% \newcommand{\en}{\mathop{\unh{n,n}-\un{n}}\nolimits}
% \newcommand{\enmu}{\mathop{\unh{n,n-1}-\un{n-1}}\nolimits}
% \newcommand{\et}{\mathop{\unh{n,n-1}-\un{n,n-1}}\nolimits}
% \newcommand{\eN}{\mathop{\unh{N,N}-\un{N}}\nolimits}
% \newcommand{\enOm}{\mathop{\unh{m,m}-\un{m}}\nolimits}
% \newcommand{\eO}{\mathop{\unh{1,0}-\un{0}}\nolimits}
%\newcommand{\eS}{\mathop{e^{n}_{h,\Dt}}\nolimits}
%
%\newcommand{\eSc}{\mathop{e_{h,\Dt}}\nolimits}
\newcommand{\eSc}{\mathop{e}\nolimits}
%
%\newcommand{\eSn}[1]{\mathop{e^{#1}_{h,\Dt}}\nolimits}
%\newcommand{\etsd}{\mathop{\epsilon^{n}_{h,\Dt}}\nolimits}
%
\newcommand{\ROnhCD}{\mathop{\duSdt-\iPe\triangle\uS+\DauS-f}\nolimits}
\newcommand{\RTnhCD}{\mathop{\left.\RonhCD\right|_T}\nolimits}
\newcommand{\RonhCD}{\mathop{R^{n}_\domO\!\!\left(t,\uS\right)}\nolimits}
\newcommand{\RtnhCD}{\mathop{R^{n}_T\!\!\left(t,\uS\right)}\nolimits}
\newcommand{\RTnhCDn}{\mathop{\left.\duSdt-\iPe\triangle\unh{n,n}+\Daunh{n}{n,n}-\fn{n}\right|_T}\nolimits}
\newcommand{\RtnhCDn}{\mathop{R^{n}_T\!\!\left(\tn{n},\unh{n,n}\right)}\nolimits}
\newcommand{\RTnhCDt}{\mathop{\left.\duSdt-\iPe\triangle\unh{n,n-1}+\Daunh{n-1}{n,n-1}-\fn{n-1}\right|_T}\nolimits}
\newcommand{\RtnhCDt}{\mathop{R^{n}_T\!\!\left(\tn{n-1},\unh{n,n-1}\right)}\nolimits}
%
\newcommand{\JEnhCD}{\mathop{\iPe\jump{\frac{\partial\uS}{\partial\n_E}}}\nolimits}
\newcommand{\JenhCD}{\mathop{J^{n}_E\!\!\left(t,\uS\right)}\nolimits}
%
\newcommand{\ROnhCal}{\mathop{\sum_{T\in\Thn{n}}\RtnhCal}\nolimits}
\newcommand{\ROsnhCal}{\mathop{\sum_{\Ts\in\Thn{n-1,n}}\RtsnhCal}\nolimits}
\newcommand{\RTnhCal}{\mathop{\left.\duSdt-\theta\kkT\triangle\unh{n,n}\!-\!(1\!-\!\theta)\kkT\triangle\unh{n,n-1}\!-\theta\Pfn{n}\!-(1\!-\!\theta)\Pfn{n-1}\right|_T}\nolimits}
\newcommand{\RTsnhCal}{\mathop{\left.\duScdt-\theta\kkTs\triangle\unh{n}\!-\!(1\!-\!\theta)\kkTs\triangle\unh{n-1}\!-\theta\Pfn{n}\!-(1\!-\!\theta)\Pfn{n-1}\right|_{\Ts}}\nolimits}
%\newcommand{\RonhCal}{\mathop{R^{n}_\domO\!\!\left(\uS\right)}\nolimits}
%\newcommand{\RosnhCal}{\mathop{R^{n}_\domO\!\!\left(\uSc\right)}\nolimits}
\newcommand{\RosnhCal}{\mathop{R^{n}_\domO}\nolimits}
%\newcommand{\RtnhCal}{\mathop{R^{n}_T\!\!\left(\uS\right)}\nolimits}
\newcommand{\RtnhCal}{\mathop{R^{n}_T}\nolimits}
%\newcommand{\RtsnhCal}{\mathop{R^{n}_{\Ts}\!\!\left(\uSc\right)}\nolimits}
\newcommand{\RtsnhCal}{\mathop{R^{n}_{\Ts}}\nolimits}
%\newcommand{\RtpnhCal}{\mathop{R^{n}_{\Tp}\!\!\left(\uSc\right)}\nolimits}
\newcommand{\RtpnhCal}{\mathop{R^{n}_{\Tp}}\nolimits}
%
\newcommand{\JEnhCal}{\mathop{\jump{{\theta}{\kkT}\frac{\partial\unh{n,n}}{\partial n_E}+(1-\theta)\kkT\frac{\partial\unh{n,n-1}}{\partial n_E}}\nolimits}}
\newcommand{\JEsnhCal}{\mathop{\jumps{{\theta}{\kkTp}\frac{\partial\unh{n}}{\partial n_{\Es}}+(1-\theta)\kkTp\frac{\partial\unh{n-1}}{\partial n_{\Es}}}\nolimits}}
%\newcommand{\JenhCal}{\mathop{J^{n}_E\!\!\left(\uS\right)}\nolimits}
\newcommand{\JenhCal}{\mathop{J^{n}_E}\nolimits}
%\newcommand{\JesnhCal}{\mathop{J^{n}_{\Es}\!\!\left(\uSc\right)}\nolimits}
\newcommand{\JesnhCal}{\mathop{J^{n}_{\Es}}\nolimits}
%
\newcommand{\DuOnhCal}{\mathop{\unh{n,n}-\unh{n,n-1}}\nolimits}
\newcommand{\DuTnhCal}{\mathop{\left.\unh{n,n}-\unh{n,n-1}\right|_T}\nolimits}
\newcommand{\NOnhCal}{\mathop{\nabla\left(\unh{n,n}-\unh{n,n-1}\right)}\nolimits}
\newcommand{\NTnhCal}{\mathop{\left.\nabla\left(\unh{n,n}-\unh{n,n-1}\right)\right|_T}\nolimits}
\newcommand{\DuOsnhCal}{\mathop{\unh{n}-\unh{n-1}}\nolimits}
\newcommand{\DuTsnhCal}{\mathop{\left.\unh{n}-\unh{n-1}\right|_T}\nolimits}
\newcommand{\NOsnhCal}{\mathop{\nabla\left(\unh{n}-\unh{n-1}\right)}\nolimits}
\newcommand{\NTsnhCal}{\mathop{\left.\nabla\left(\unh{n}-\unh{n-1}\right)\right|_{\Ts}}\nolimits}
%
\newcommand{\taunT}[1]{\mathop{\tau^{#1}_T}\nolimits}
\newcommand{\PenT}[1]{\mathop{Pe^{#1}_T}\nolimits}
%
\newcommand{\EHn}{\mathop{\CAL{E}^{n}_{h}}\nolimits}
\newcommand{\EOn}{\mathop{\CAL{E}^{n}_{h,\domO}}\nolimits}
\newcommand{\EGn}{\mathop{\CAL{E}^{n}_{h,\partial\domO}}\nolimits}
%
\newcommand{\Ehn}[1]{\mathop{\CAL{E}^{#1}_{h}}\nolimits}
\newcommand{\Eon}[1]{\mathop{\CAL{E}^{#1}_{h,\domO}}\nolimits}
\newcommand{\Egn}[1]{\mathop{\CAL{E}^{#1}_{h,\partial\domO}}\nolimits}
%
\newcommand{\Errn}{\mathop{E^{n}_{h,\Dt}}\nolimits}
\newcommand{\deSdt}{\mathop{\frac{\partial\eS}{\partial t}}\nolimits}
\newcommand{\deScdt}{\mathop{\frac{\partial\eSc}{\partial t}}\nolimits}
\newcommand{\deScdtt}{\mathop{\frac{\partial\eSc(t)}{\partial t}}\nolimits}
\newcommand{\DaeS}{\mathop{\Va\cdot\nabla\eS}\nolimits}
\newcommand{\intn}[1]{\mathop{\int_{\tn{n\!-\!1}}^{\tn{n}} #1\!\diff
t}\nolimits}
\newcommand{\intOm}[1]{\mathop{\ds\sum_{n=1}^m\intn{#1}}\nolimits}
\newcommand{\intON}[1]{\mathop{\int_{0}^{\Xi} #1\!\diff t}\nolimits}
%\newcommand{\IeS}{\mathop{I_h e^{n}_{h,\Dt}}\nolimits}
%\newcommand{\IeSc}{\mathop{I_h e_{h,\Dt}}\nolimits}
%\newcommand{\DaIeS}[1]{\mathop{\Va^{#1}\cdot\nabla \IeS}\nolimits}
\newcommand{\Iv}{\mathop{I_h v}\nolimits}
%
\newcommand{\etaRTn}{\mathop{{
	\eta^{n}_{R,T}}}\nolimits}
\newcommand{\etaNABLATn}{\mathop{{
	\eta^{n}_{\nabla,T}}}\nolimits}
%
\newcommand{\etaRTnq}{\mathop{{
	\left(\eta^{n}_{R,T}\right)^2}}\nolimits}
\newcommand{\etaNABLATnq}{\mathop{{
	\left(\eta^{n}_{\nabla,T}\right)^2}}\nolimits}
%
\newcommand{\etaRTsn}{\mathop{{
	\eta^{n}_{R,\Ts}}}\nolimits}
\newcommand{\etaNABLATsn}{\mathop{{
	\eta^{n}_{\nabla,\Ts}}}\nolimits}
%
\newcommand{\etaRTsnq}{\mathop{{
	\left(\eta^{n}_{R,\Ts}\right)^2}}\nolimits}
\newcommand{\etaNABLATsnq}{\mathop{{
	\left(\eta^{n}_{\nabla,\Ts}\right)^2}}\nolimits}
%
\newcommand{\etaATnq}{\mathop{{
	\left(\eta^{n}_{\Va,T}\right)^2}}\nolimits}
\newcommand{\etaFTnq}{\mathop{{
	\left(\eta^{n}_{f,T}\right)^2}}\nolimits}
\newcommand{\etaRTnqMax}{\mathop{{
	\left(\eta^{n}_{R,T,MAX}\right)^2}}\nolimits}
\newcommand{\etaRTnqmin}{\mathop{{
	\left(\eta^{n}_{R,T,min}\right)^2}}\nolimits}
\newcommand{\etaRTnqrms}{\mathop{\sigma_{\etaRTnq}}\nolimits}
%
\newcommand{\etatotTnq}{\mathop{{
	\left(\eta^{n}_{tot,T}\right)^2}}\nolimits}
\newcommand{\fetatotTnq}[1]{\mathop{{
	\left(\eta^{n}_{\rm tot,T}\!\left({#1}\right)\right)^2}}\nolimits}
\newcommand{\etatotnq}{\mathop{{
	\left(\eta^{n}_{tot}\right)^2}}\nolimits}
\newcommand{\etatotq}{\mathop{{
	\left(\eta_{tot}\right)^2}}\nolimits}
%
\newcommand{\etaRnq}{\mathop{{
	\left(\eta^{n}_{R}\right)^2}}\nolimits}
\newcommand{\etaNABLAnq}{\mathop{{
	\left(\eta^{n}_{\nabla}\right)^2}}\nolimits}
\newcommand{\etaAnq}{\mathop{{
	\left(\eta^{n}_{\Va}\right)^2}}\nolimits}
\newcommand{\etaFnq}{\mathop{{
	\left(\eta^{n}_{f}\right)^2}}\nolimits}
\newcommand{\etaFntq}{\mathop{{
	\left(\eta^{n}_{f,\theta,\Dtn}\right)^2}}\nolimits}
\newcommand{\etaFnxq}{\mathop{{
	\left(\eta^{n}_{f,\PrT}\right)^2}}\nolimits}
\newcommand{\etaFtq}{\mathop{{
	\eta^2_{f,\theta,\Dtn}}}\nolimits}
\newcommand{\etaFxq}{\mathop{{
	\eta^2_{f,\PrT}}}\nolimits}
\newcommand{\etaTOTnq}{\mathop{{
	\left(\eta^{n}_{\rm tot}\right)^2}}\nolimits}
%
\newcommand{\etaRq}{\mathop{\eta^2_{R}}\nolimits}
\newcommand{\etaNABLAq}{\mathop{\eta^2_{\nabla}}\nolimits}
\newcommand{\etaAq}{\mathop{\eta^2_{\Va}}\nolimits}
\newcommand{\etaFq}{\mathop{\eta^2_{f}}\nolimits}
%
\newcommand{\etaRn}{\mathop{{\eta^{n}_{R}}}\nolimits}
\newcommand{\etaNABLAn}{\mathop{{\eta^{n}_{\nabla}}}\nolimits}
\newcommand{\etaAn}{\mathop{{\eta^{n}_{\Va}}}\nolimits}
\newcommand{\etaTOTn}{\mathop{{\eta^{n}_{\rm tot}}}\nolimits}
\newcommand{\etaFn}{\mathop{{\eta^{n}_{f}}}\nolimits}
\newcommand{\etaFnt}{\mathop{{
	\eta^{n}_{f,\theta,\Dtn}}}\nolimits}
\newcommand{\etaFnx}{\mathop{{
	\eta^{n}_{f,\PrT}}}\nolimits}
%
%\newcommand{\errnormdef}{\mathop{\enorm{\eS}{\kk,(a,b)}}\nolimits}
%\newcommand{\errnorm}{\mathop{\enorm{\eS}{\kk,(\tn{n-1},\tn{n})}}\nolimits}
\newcommand{\errnorm}{\mathop{\enorm{\eS}{\kk,\InC}}\nolimits}
\newcommand{\errcnorm}{\mathop{\enorm{\eSc}{\kk,\InC}}\nolimits}
%\newcommand{\errnormq}{\mathop{\enormn{\eS}{\kk,(\tn{n-1},\tn{n})}{2}}\nolimits}
\newcommand{\errnormq}{\mathop{\enormn{\eS}{\kk,\InC}{2}}\nolimits}
\newcommand{\errcnormq}{\mathop{\enormn{\eSc}{\kk,\InC}{2}}\nolimits}
%\newcommand{\errnormON}{\mathop{\enorm{\eS}{\kk,(0,\Xi)}}\nolimits}
%\newcommand{\errnormONq}{\mathop{\enormn{\eS}{\kk,(0,\Xi)}{2}}\nolimits}
%
\newcommand{\errnormOm}{\mathop{\enorm{\eS}{\kk,(0,\tn{m})}}\nolimits}
\newcommand{\errnormOmq}{\mathop{\enormn{\eS}{\kk,(0,\tn{m})}{2}}\nolimits}
\newcommand{\errcnormOm}{\mathop{\enorm{\eSc}{\kk,(0,\tn{m})}}\nolimits}
\newcommand{\errcnormOmq}{\mathop{\enormn{\eSc}{\kk,(0,\tn{m})}{2}}\nolimits}
%
%\newcommand{\CDtn}[2]{\mathop{\VEC{C}_{#1}^{#2}}\nolimits}
\newcommand{\Cen}[2]{\mathop{C_{#1}^{#2}}\nolimits}
\newcommand{\Cten}[2]{\mathop{\tilde{C}_{#1}^{#2}}\nolimits}
\newcommand{\Ctten}[2]{\mathop{\tilde{\tilde{C}}_{#1}^{#2}}\nolimits}
\newcommand{\Cbelow}[2]{\mathop{C_{\downarrow,#1}^{#2}}\nolimits}
\newcommand{\Cabove}[2]{\mathop{C_{#1}^{\uparrow,#2}}\nolimits}
\newcommand{\Ctabove}[2]{\mathop{\tilde{C}_{#1}^{\uparrow,#2}}\nolimits}
\newcommand{\cten}[2]{\mathop{\tilde{c}_{#1}^{#2}}\nolimits}
\newcommand{\ctten}[2]{\mathop{\tilde{\tilde{c}}_{#1}^{#2}}\nolimits}
%\newcommand{\cbelow}[2]{\mathop{c_{\downarrow,[#1]}^{#2}}\nolimits}
%\newcommand{\cabove}[2]{\mathop{c_{#1}^{\uparrow,[#2]}}\nolimits}
%
\newcommand{\bn}{\mathop{b^{n}}\nolimits}
\newcommand{\bTn}{\mathop{b^{n}_{T}}\nolimits}
\newcommand{\bEn}{\mathop{b^{n}_{E}}\nolimits}
\newcommand{\bTsn}{\mathop{b^{n}_{\Ts}}\nolimits}
\newcommand{\bEsn}{\mathop{b^{n}_{\Es}}\nolimits}
\newcommand{\bTs}{\mathop{b_{\Ts}}\nolimits}
\newcommand{\bEs}{\mathop{b_{\Es}}\nolimits}
%
\newcommand{\wnT}{\mathop{w^{n}_{R,T}}\nolimits}
\newcommand{\wnTs}{\mathop{w^{n}_{R,\Ts}}\nolimits}
\newcommand{\wnRO}{\mathop{w^{n}_{R,\domO}}\nolimits}
%\newcommand{\bnR}{\mathop{b^{n}_{R}}\nolimits}
\newcommand{\bnR}{\mathop{\bn}\nolimits}
\newcommand{\dwnTdt}{\mathop{\frac{\partial \wnT}{\partial t}}\nolimits}
\newcommand{\dwnROdt}{\mathop{\frac{\partial \wnRO}{\partial t}}\nolimits}
%
%\newcommand{\wkTs}{\mathop{w^{[k_{\Ts}]}_{R,\Ts}}\nolimits}
\newcommand{\wkNTs}{\mathop{w^{k_{\Ts}}_{\nabla,\Ts}}\nolimits}
\newcommand{\wkEsNO}{\mathop{w^{k_{\Es}}_{\nabla,\domO}}\nolimits}
%
\newcommand{\wnNT}{\mathop{w^{n}_{\nabla,T}}\nolimits}
\newcommand{\wnNO}{\mathop{w^{n}_{\nabla,\domO}}\nolimits}
%
\newcommand{\wnE}{\mathop{w^{n}_{J,E}}\nolimits}
\newcommand{\wnEs}{\mathop{w^{n}_{J,\Es}}\nolimits}
\newcommand{\wnJO}{\mathop{w^{n}_{J,\domO}}\nolimits}
%\newcommand{\bnE}{\mathop{b^{n}_{E}}\nolimits}
\newcommand{\bnE}{\mathop{\bn}\nolimits}
\newcommand{\dwnEdt}{\mathop{\frac{\partial \wnE}{\partial t}}\nolimits}
\newcommand{\dwnJOdt}{\mathop{\frac{\partial \wnJO}{\partial t}}\nolimits}
%
\newcommand{\va}[1]{\mathop{\VEC{a}_{#1}}\nolimits}
\newcommand{\Tu}{\mathop{T^{\upt}}\nolimits}
\newcommand{\Td}{\mathop{T^{\downt}}\nolimits}
\newcommand{\Tud}{\mathop{T^{\upt}_2}\nolimits}
\newcommand{\Tdd}{\mathop{T^{\downt}_2}\nolimits}
%\newcommand{\oEd}{\mathop{\omega_{E,2}}\nolimits}
\newcommand{\oEd}{\mathop{\stackrel{_\diamond}{\omega}_{E}}\nolimits}
%
\newcommand{\oTn}{\mathop{\omega_T^{n}}\nolimits}
\newcommand{\oTtn}{\mathop{\tilde{\omega}_T^{n}}\nolimits}
\newcommand{\oEn}{\mathop{\omega_E^{n}}\nolimits}
\newcommand{\oEtn}{\mathop{\tilde{\omega}_E^{n}}\nolimits}
\newcommand{\oEdn}{\mathop{\stackrel{_\diamond}{\omega}_{E}^{n}}\nolimits}
%
\newcommand{\oTsn}{\mathop{\omega_{\Ts}^{n}}\nolimits}
\newcommand{\oTstn}{\mathop{\tilde{\omega}_{\Ts}^{n}}\nolimits}
\newcommand{\oEsn}{\mathop{\omega_{\Es}^{n}}\nolimits}
\newcommand{\oEstn}{\mathop{\tilde{\omega}_{\Es}^{n}}\nolimits}
\newcommand{\oEsdn}{\mathop{\stackrel{_\diamond}{\omega}_{\Es}^{n}}\nolimits}
%
\newcommand{\UCDnormrefn}{\mathop{
	\ds\intn{\iPe\normn{\nabla\uS}{0}{2}}}\nolimits}
\newcommand{\UCDnormrefON}{\mathop{
	\ds\intON{\iPe\normn{\nabla\uS}{0}{2}}}\nolimits}
\newcommand{\ucdnormrefn}[1]{\mathop{\enorm{#1}{{n,\sobho{1}{\domO}}}\nolimits}}
\newcommand{\ucdnormrefnn}[2]{\mathop{\enormn{#1}{{n,\sobho{1}{\domO}}}{#2}\nolimits}}
%
\newcommand{\sigmaT}{\mathop{{\sigma_{_{T}}}}\nolimits}
%
%
%
\newcommand{\euno}{\mathop{\unh{1,0}-\un{0}}\nolimits}
\newcommand{\etaRnquno}{\mathop{{
	\left(\eta^{[1]}_{R}\right)^2}}\nolimits}
\newcommand{\etaNABLAnquno}{\mathop{{
	\left(\eta^{[1]}_{\nabla}\right)^2}}\nolimits}
\newcommand{\etaFnquno}{\mathop{{
	\left(\eta^{[1]}_{f}\right)^2}}\nolimits}
\newcommand{\IunoC}{\mathop{I^{1}}\nolimits}
\newcommand{\errnormquno}{\mathop{\enormn{\eSn{1}}{\kk,\IunoC}{2}}\nolimits}
%
%
%
\newcommand{\ute}{\mathop{{u.t.e.}^{n}}\nolimits}
\newcommand{\lte}{\mathop{{l.t.e.}^{n}}\nolimits}
\newcommand{\uee}{\mathop{{u.e.e.}^{n}}\nolimits}
\newcommand{\lee}{\mathop{{l.e.e.}^{n}}\nolimits}
%
\newcommand{\uteq}{\mathop{\left({u.t.e.}^{n}\right)^2}\nolimits}
\newcommand{\lteq}{\mathop{\left({l.t.e.}^{n}\right)^2}\nolimits}
\newcommand{\ueeq}{\mathop{\left({u.e.e.}^{n}\right)^2}\nolimits}
\newcommand{\leeq}{\mathop{\left({l.e.e.}^{n}\right)^2}\nolimits}
%
\newcommand{\normdedtn}{\mathop{\varepsilon_{\kk,-1}^{n}}\nolimits}
\newcommand{\normen}{\mathop{\varepsilon_{\kk,1}^{n}}\nolimits}
\newcommand{\normdedtnq}{\mathop{\left(\varepsilon_{\kk,-1}^{n}\right)^2}\nolimits}
\newcommand{\normenq}{\mathop{\left(\varepsilon_{\kk,1}^{n}\right)^2}\nolimits}
%
\newcommand{\unormq}{\mathop{\enormn{\uSc}{\kk,\InC}{2}}\nolimits}
%
%
%
%
%\newcommand{\dudtxt}{\mathop{\frac{\partial u}{\partial t}(x,t)}\nolimits}
%\newcommand{\uScxt}{\mathop{u_{h,\Dt}(x,t)}\nolimits}
\newcommand{\dudtxt}{\mathop{\frac{\partial u}{\partial t}(t)}\nolimits}
\newcommand{\uScxt}{\mathop{u_{h,\Dt}(t)}\nolimits}
\newcommand{\duScdtxt}{\mathop{\frac{\partial\uScxt}{\partial t}}\nolimits}
\newcommand{\duScdtt}{\mathop{\frac{\partial\uSc(t)}{\partial t}}\nolimits}
%
%\newcommand{\eScxt}{\mathop{e_{h,\Dt}(x,t)}\nolimits}
%\newcommand{\eScxt}{\mathop{e_{h,\Dt}(t)}\nolimits}
\newcommand{\eScxt}{\mathop{\eSc(t)}\nolimits}
\newcommand{\deScdtxt}{\mathop{\frac{\partial\eScxt}{\partial t}}\nolimits}
%
\newcommand{\upn}[1]{\mathop{u_{p}^{{#1}}}\nolimits}
\newcommand{\phipn}[1]{\mathop{\phi^{{#1}}}\nolimits}
\newcommand{\vphipn}[1]{\mathop{\varphi_{p}^{#1}}\nolimits}
\newcommand{\vphippn}[1]{\mathop{\varphi_{p'}^{#1}}\nolimits}
\newcommand{\vphipr}{\mathop{\varphi_{p_r}^{n-1,n}}\nolimits}
\newcommand{\tpn}[1]{\mathop{t^{{#1}}}\nolimits}
\newcommand{\IpnC}{\mathop{[\tpn{n,k_p-1},\tpn{n,k_p}]}\nolimits}
%\newcommand{\IpnCmax}{\mathop{[\tpn{\Jpn,k_p-1},\tpn{\Jpn,k_p}]}\nolimits}
\newcommand{\ITnC}{\mathop{[\tpn{n,k_T-1},\tpn{n,k_T}]}\nolimits}
\newcommand{\ITnc}{\mathop{[\tpn{k_T-1},\tpn{k_T}]}\nolimits}
\newcommand{\ITnCs}{\mathop{[\tpn{k_{\Ts}-1},
        \tpn{k_{\Ts}}]}\nolimits}
\newcommand{\ITns}{\mathop{\left(\tpn{k_{\Ts}-1},
        \tpn{k_{\Ts}}\right)}\nolimits}
\newcommand{\IEnCs}{\mathop{[\tpn{k_{\Es}-1},
        \tpn{k_{\Es}}]}\nolimits}
\newcommand{\chipn}[1]{\mathop{\chi_{p}^{#1}}\nolimits}
\newcommand{\chikp}{\mathop{\chi_{k_p}}\nolimits}
\newcommand{\chik}[1]{\mathop{\chi_{#1-1}^{#1}}\nolimits}
\newcommand{\chiTsk}{\mathop{\chi_{k_{\Ts}\!-1}^{k_{\Ts}}}\nolimits}
\newcommand{\chiTk}{\mathop{\chi_{k_{T}\!-1}^{k_{T}}}\nolimits}
%
\newcommand{\Prn}{\mathop{\Pi^{n}}\nolimits}
\newcommand{\Pfpn}[1]{\mathop{{\Prn\!f(x,\tpn{#1})}}\nolimits}
%
\newcommand{\Whn}[1]{\mathop{{\rm W}_h^{#1}}\nolimits}
%
%\newcommand{\PrTh}{\mathop{\Pi_{\Thn{n}}}\nolimits}
\newcommand{\PrTh}{\mathop{\Pi_{h}^{n}}\nolimits}
\newcommand{\PrThfn}[1]{\mathop{{\PrTh\!\fn{#1}}}\nolimits}
%
\newcommand{\fSc}{\mathop{f_{h,\Dt}}\nolimits}
\newcommand{\fkTs}{\mathop{\IVhnDtn\fSc}\nolimits}
%
\newcommand{\intkT}[1]{\mathop{
        \int_{\tpn{n,k_T-1}}^{\tpn{n,k_T}} #1\!\diff t
        }\nolimits}
%\newcommand{\intkE}[1]{\mathop{
%        \int_{\tpn{\JEsn,k_{\Es}-1}}^{\tpn{\JEsn,k_{\Es}}} #1\!\diff t
%        }\nolimits}
%
\newcommand{\Ts}{\mathop{T_{\!^{*}}}\nolimits}
\newcommand{\Tp}{\mathop{T'}\nolimits}
\newcommand{\Es}{\mathop{E_{\!{*}}}\nolimits}
\newcommand{\intkTs}[1]{\mathop{
        \int_{\tpn{k_{\Ts}\!\!-1}}^{\tpn{k_{\Ts}}} #1\!\diff t
        }\nolimits}
\newcommand{\intkEs}[1]{\mathop{
        \int_{\tpn{k_{\Es}-1}}^{\tpn{k_{\Es}}} #1\!\diff t
        }\nolimits}
\newcommand{\intJ}[1]{\mathop{
        \int_{\tpn{n,J,k-1}}^{\tpn{n,J,k}} #1\!\diff t
        }\nolimits}
\newcommand{\intkJ}[1]{\mathop{
        \int_{\tpn{k-1}}^{\tpn{k}} #1\!\diff t
        }\nolimits}
\newcommand{\DtnTs}{\mathop{\Dt_{\Ts}}\nolimits}
\newcommand{\DtnTp}{\mathop{\Dt_{\Tp}}\nolimits}
\newcommand{\DtnEs}{\mathop{\Dt_{\Es}}\nolimits}
%
%\newcommand{\RtsnhCals}{\mathop{R^{[n,j_{\Ts},k_{\Ts}]}_{\Ts}}\nolimits}
\newcommand{\RtsnhCals}{\mathop{R^{k_{\Ts}}_{\Ts}}\nolimits}
\newcommand{\RtsnhCalss}{\mathop{R^{k_{\Ts}}_{\Ts}}\nolimits}
\newcommand{\RtsnhCalssEs}{\mathop{R^{k_{\Es}}_{T'}}\nolimits}
\newcommand{\RtpnhCals}{\mathop{R^{n,j_{\Tp},k_{\Tp}}_{\Tp}}\nolimits}
\newcommand{\rOsnhCalss}{\mathop{r^{n}_{\domO}(v_h)}\nolimits}
\newcommand{\rOv}[1]{\mathop{r^{n}_{\domO}(#1)}\nolimits}
\newcommand{\rTsv}[1]{\mathop{r^{n}_{\Ts}(#1)}\nolimits}
\newcommand{\rO}{\mathop{r^{n}_{\domO}}\nolimits}
\newcommand{\rOk}{\mathop{r^{k}_{\domO}}\nolimits}
\newcommand{\rOkv}[1]{\mathop{r^{k}_{\domO}(#1)}\nolimits}
%
\newcommand{\JEsnhCalS}{\mathop{
\jumps{{\oot}{\kkTp}\frac{\partial\uSc(x,\tpn{n,j_{\Es},k_{\Es}})}
{\partial n_{\Es}}
+\oot\kkTp\frac{\partial\uSc(x,\tpn{n,j_{\Es},k_{\Es}-1})}
{\partial n_{\Es}}}\nolimits}}
\newcommand{\JEsnhCals}{\mathop{
\jumps{\frac{\kkTp}{2}
\frac{\partial(\uSc(\tpn{k_{\Es}})+\uSc(\tpn{k_{\Es}-1}))}
{\partial n_{\Es}}}
\nolimits}}
% \newcommand{\DuDnEsnhCals}{\mathop{
% {\oot}{\kk}\frac{\partial\uSc(x,\tpn{n,j_{\Es},k_{\Es}})}
% {\partial n_{\Es}}
% +\oot\kk\frac{\partial\uSc(x,\tpn{n,j_{\Es},k_{\Es}-1})}
% {\partial n_{\Es}}}\nolimits}
% \newcommand{\dudnesnhCals}{\mathop{\frac{\delta u_{h,\Dt}^{[k_{\Es}]}}
% {\delta n_{\Es}}}\nolimits}
% \newcommand{\dudnesnhCalss}{\mathop{\frac{\delta u_{h,\Dt}^{[k'_{\Es}]}}
% {\delta n_{\Es}}}\nolimits}
\newcommand{\JesnhCals}{\mathop{J^{k_{\Es}}_{\Es}}\nolimits}
\newcommand{\JesnhCalss}{\mathop{J^{k_{\Es}}_{\Es}}\nolimits}
%
\newcommand{\etaRTskqs}{\mathop{{
	\left(\eta^{k_{\Ts}}_{R,\Ts}\right)^2}}\nolimits}
\newcommand{\etaRTsnqs}{\mathop{{
	\left(\eta^{n}_{R,\Ts}\right)^2}}\nolimits}
\newcommand{\etaNABLATsnqs}{\mathop{{
	\left(\eta^{n}_{\nabla,\Ts}\right)^2}}\nolimits}
\newcommand{\etaNABLATskqs}{\mathop{{
	\left(\eta^{k_{\Ts}}_{\nabla,\Ts}\right)^2}}\nolimits}
\newcommand{\etaNABLATsks}{\mathop{{
	\left(\eta^{k_{\Ts}}_{\nabla,\Ts}\right)}}\nolimits}
%
% \newcommand{\etaFntqs}{\mathop{{
% 	\left(\eta^{n}_{f,\Dtn}\right)^2}}\nolimits}
% \newcommand{\etaFnxqs}{\mathop{{
% 	\left(\eta^{n}_{f,\PrTh}\right)^2}}\nolimits}
\newcommand{\etaFntqs}{\mathop{{
	\left(\eta^{n}_{f,\Dt}\right)^2}}\nolimits}
\newcommand{\etaFnxqs}{\mathop{{
	\left(\eta^{n}_{f,\Pi_{h}}\right)^2}}\nolimits}
%\newcommand{\etaFnts}{\mathop{{
%	\eta^{n}_{f,\Dtn}}}\nolimits}
%\newcommand{\etaFnxs}{\mathop{{
%	\eta^{n}_{f,\PrTh}}}\nolimits}
\newcommand{\etaFnts}{\mathop{{
	\eta^{n}_{f,\Dt}}}\nolimits}
\newcommand{\etaFnxs}{\mathop{{
	\eta^{n}_{f,\Pi_{h}}}}\nolimits}
%
\newcommand{\etaDeltaTskqs}{\mathop{{
	\left(\eta^{k_{\Ts}}_{\delta,\Ts}\right)^2}}\nolimits}
\newcommand{\etaDeltaTsnqs}{\mathop{{
	\left(\eta^{n}_{\delta,\Ts}\right)^2}}\nolimits}
%
\newcommand{\etaDeltasnqs}{\mathop{{
	\left(\eta^{n}_{\delta}\right)^2}}\nolimits}
\newcommand{\etaDeltasn}{\mathop{{\eta^{n}_{\delta}}}\nolimits}
%
\newcommand{\etaDeltasnqsmin}{\mathop{{
	\left(\eta^{n}_{\delta,min}\right)^2}}\nolimits}
\newcommand{\etaDeltasnqsmid}{\mathop{{
	\left(\eta^{n}_{\delta,mid}\right)^2}}\nolimits}
\newcommand{\etaDeltasnqsMAX}{\mathop{{
	\left(\eta^{n}_{\delta,MAX}\right)^2}}\nolimits}
\newcommand{\etaDeltasnsmin}{\mathop{{
	\eta^{n}_{\delta,min}}}\nolimits}
\newcommand{\etaDeltasnsmid}{\mathop{{
	\eta^{n}_{\delta,mid}}}\nolimits}
\newcommand{\etaDeltasnsMAX}{\mathop{{
	\eta^{n}_{\delta,MAX}}}\nolimits}
%
\newcommand{\etadufsnqs}{\mathop{{
	\left(\eta^{n}_{\partial u,f}\right)^2}}\nolimits}
%
\newcommand{\Vhntr}[1]{\mathop{{\rm V}_{h,tr}^{#1}}\nolimits}
\newcommand{\Vhncn}[1]{\mathop{{\rm V}_{h,cn}^{#1}}\nolimits}
%\newcommand{\VhnB}[1]{\mathop{{\rm V}_{h,B}^{#1}}\nolimits}
%
%\newcommand{\IVhn}{\mathop{{I_{\Vhn{n}}}}\nolimits}
\newcommand{\IVhn}{\mathop{{I_{h}^{n}}}\nolimits}
%\newcommand{\IVhntr}{\mathop{{I_{\Vhntr{n}}}}\nolimits}
\newcommand{\IVhntr}{\mathop{{I_{h}^{n}}}\nolimits}
%
%\newcommand{\IVhnB}{\mathop{{I_{\VhnB{n}}}}\nolimits}
%\newcommand{\IDtn}{\mathop{{I_{\Dtn}}}\nolimits}
%\newcommand{\IVhnDtn}{\mathop{{I_{\Vhn{n},\Dtn}}}\nolimits}
%
%\newcommand{\IheSc}{\mathop{\IVhn e_{h,\Dt}}\nolimits}
\newcommand{\IheSc}{\mathop{\IVhn\!\eSc}\nolimits}
%
%\newcommand{\IhtreSc}{\mathop{\IVhntr e_{h,\Dt}}\nolimits}
%\newcommand{\IhBeSc}{\mathop{\IVhnB e_{h,\Dt}}\nolimits}
%\newcommand{\IhIDteSc}{\mathop{\IVhnDtn e_{h,\Dt}}\nolimits}
%
\newcommand{\vcnorm}{\mathop{\enorm{v}{\kk,\InC}}\nolimits}
%
\newcommand{\bkTs}{\mathop{b^{k_{\Ts}}}\nolimits}
\newcommand{\bkEs}{\mathop{b^{k_{\Es}}}\nolimits}
\newcommand{\wkTs}{\mathop{w^{k_{\Ts}}_{R,\Ts}}\nolimits}
\newcommand{\wkEs}{\mathop{w^{k_{\Es}}_{J,\Es}}\nolimits}
%
\newcommand{\wnNTs}{\mathop{w^{k_{\Ts}}_{\nabla,\Ts}}\nolimits}
%\newcommand{\wnNO}{\mathop{w^{n}_{\nabla,\domO}}\nolimits}
\newcommand{\NTsnhCals}{\mathop{
\nabla\uSc(x,\tpn{k_{\Ts}})-\uSc(x,\tpn{k_{\Ts}-1})
}\nolimits}
\newcommand{\DuTsnhCals}{\mathop{
\uSc(x,\tpn{k_{\Ts}})-\uSc(x,\tpn{k_{\Ts}-1})
}\nolimits}
%
\newcommand{\opn}{\mathop{\omega_p^{n}}\nolimits}
\newcommand{\eScp}{\mathop{e_{h,\Dt,p}}\nolimits}
%
\newcommand{\DtT}{\mathop{\Delta\!t_T}\nolimits}
\newcommand{\DtTs}{\mathop{\Delta\!t_{\Ts}}\nolimits}
\newcommand{\DtTp}{\mathop{\Delta\!t_{T'}}\nolimits}
\newcommand{\DtEs}{\mathop{\Delta\!t_{\Es}}\nolimits}
\newcommand{\DtJ}{\mathop{\Delta\!t_J}\nolimits}
\newcommand{\Dtp}{\mathop{\Delta\!t_p}\nolimits}
%
\newcommand{\intk}[1]{\mathop{
        \int_{\tpn{k-1}}^{\tpn{k}} #1\!\diff t
        }\nolimits}
%
\newcommand{\uScc}{\mathop{\bar{u_{h,\Dt}}}\nolimits}
\newcommand{\duSccdt}{\mathop{\frac{\partial\uScc}{\partial
        t}}\nolimits}
%
\newcommand{\EHdn}[2]{\mathop{\CAL{E}^{#2}_{h,#1}}\nolimits}
\newcommand{\eSt}{\mathop{e_{\Dt}}\nolimits}
%
\newcommand{\chitkT}{\mathop{\chi_{_{k_{_{T}}}}\!\!\!(t)}\nolimits}
%
\newcommand{\chitk}{\mathop{\chi_{_{k_{_{{\Ts}}}}}\!\!\!(t)}\nolimits}
\newcommand{\chitkE}{\mathop{\chi_{_{k_{_{\Es}}}}\!\!\!(t)}\nolimits}
\newcommand{\chiTn}{\mathop{\chi^{n}_{T}}\nolimits}
\newcommand{\chiT}{\mathop{\chi_{_T}}\nolimits}
\newcommand{\chiTsn}{\mathop{\chi^{n}_{\Ts}}\nolimits}
%\newcommand{\chiTsx}{\mathop{\chi_{_{\Ts}}\!(x)}\nolimits}
\newcommand{\chiTsx}{\mathop{\chi_{_{\Ts}}}\nolimits}
\newcommand{\chiTs}{\mathop{\chi_{_{\Ts}}}\nolimits}
\newcommand{\normrO}{\mathop{\left\|\rO\right\|_{\kk,-1,\Th}}\nolimits}
\newcommand{\normrOk}{\mathop{\left\|\rOk\right\|_{\kk,-1,\Th}}\nolimits}
\newcommand{\normrOq}{\mathop{\left\|\rO\right\|_{\kk,-1,\Th}^2}\nolimits}
\newcommand{\normrOkq}{\mathop{\left\|\rOk\right\|_{\kk,-1,\Th}^2}\nolimits}
\newcommand{\normrOkminq}{\mathop{\left\|r^{k_{min}}_{\domO}\right\|_{\kk,-1,\Th}^2}\nolimits}
\newcommand{\normrOkmidq}{\mathop{\left\|r^{k_{mid}}_{\domO}\right\|_{\kk,-1,\Th}^2}\nolimits}
\newcommand{\normrOkMaxq}{\mathop{\left\|r^{k_{MAX}}_{\domO}\right\|_{\kk,-1,\Th}^2}\nolimits}
\newcommand{\NTskhCalss}{\mathop{\nabla\!\left(\uSc(\tpn{k_{\Ts}})\!-\!\uSc(\tpn{k_{\Ts}\!-\!1})\right)}\nolimits}
\newcommand{\DuTskhCalss}{\mathop{\uSc(\tpn{k_{\Ts}})-\uSc(\tpn{k_{\Ts}-1})}\nolimits}
\newcommand{\DuEskhCalss}{\mathop{\uSc(\tpn{k_{\Es}})-\uSc(\tpn{k_{\Es}-1})}\nolimits}
\newcommand{\MuTskhCalss}{\mathop{\frac{\uSc(\tpn{k_{\Ts}})+\uSc(\tpn{k_{\Ts}-1})}{2}}\nolimits}
%
\newcommand{\Jpn}{\mathop{J_p^{n}}\nolimits}
\newcommand{\JpnMax}{\mathop{J_{p_{Max}}^{n}}\nolimits}
\newcommand{\Jpnm}{\mathop{J_p^{n-1}}\nolimits}
\newcommand{\Jpnn}[1]{\mathop{J_p^{#1}}\nolimits}
\newcommand{\Jprn}{\mathop{J_{p_r}^{n-1,n}}\nolimits}
\newcommand{\Jprnmax}{\mathop{\hat{J}_{p_r}^{n}}\nolimits}
\newcommand{\Jppn}{\mathop{J_{p'}^{n}}\nolimits}
%
\newcommand{\JTn}{\mathop{J_T^{n}}\nolimits}
\newcommand{\JTsn}{\mathop{J_{\Ts}^{n}}\nolimits}
\newcommand{\JEsn}{\mathop{J_{\Es}^{n}}\nolimits}
\newcommand{\JTs}{\mathop{J_{\Ts}}\nolimits}
\newcommand{\JEs}{\mathop{J_{\Es}}\nolimits}
\newcommand{\Uhn}[1]{\mathop{{\rm U}_{h,\Dt}^{#1}}\nolimits}
\newcommand{\cVhn}[1]{\mathop{{\CAL V}_{h,\Dt}^{#1}}\nolimits}
\newcommand{\nuhn}{\mathop{{\nu}_{h,\Dt}}\nolimits}
\newcommand{\muhn}{\mathop{{\mu}_{h,\Dt}^{n}}\nolimits}
%
\newcommand{\uhn}{\mathop{u^{n}_{h}}\nolimits}
\newcommand{\uho}{\mathop{u^{1}_{h}}\nolimits}
\newcommand{\duhndt}{\mathop{\frac{\partial\uhn}{\partial t}}\nolimits}
\newcommand{\PrDtn}{\mathop{\Pi^{n}_{\DtT}}\nolimits}
\newcommand{\dPrDtnuhndt}{\mathop{\frac{\partial\PrDtn\uhn}{\partial t}}\nolimits}
\newcommand{\etahn}{\mathop{\eta^{n}_{h}}\nolimits}
%
\newcommand{\deltahn}{\mathop{\delta^{n}_{h}}\nolimits}
\newcommand{\xihn}{\mathop{\xi^{n}_{h}}\nolimits}
\newcommand{\xihnp}{\mathop{\xi^{n}_{h,p}}\nolimits}
\newcommand{\ehn}{\mathop{\rho^{n}_{h}}\nolimits}
\newcommand{\sigmahn}{\mathop{\sigma^{n}_{h}}\nolimits}
\newcommand{\ddeltahndt}{
\mathop{\frac{\partial\deltahn}{\partial t}}\nolimits
}
\newcommand{\dxihndt}{
\mathop{\frac{\partial\xihn}{\partial t}}\nolimits
}
\newcommand{\dxihnpdt}{
\mathop{\frac{\partial\xihnp}{\partial t}}\nolimits
}
\newcommand{\dsigmahndt}{
\mathop{\frac{\partial\sigmahn}{\partial t}}\nolimits
}
%
\newcommand{\IDtp}{\mathop{{I_{\Dtp}}}\nolimits}
\newcommand{\dIDtpuhndt}{
\mathop{\frac{\partial\IDtp\uhn}{\partial t}}\nolimits}
\newcommand{\IkTC}{\mathop{I^{k_T}}\nolimits}
%\newcommand{\IkTsC}{\mathop{I^{[k_{\Ts}]}}\nolimits}
\newcommand{\DtpT}{\mathop{\Delta\!t_{p,T}}\nolimits}
\newcommand{\intkp}[1]{\mathop{
        \int_{\tpn{\Jpn,k_p-1}}^{\tpn{\Jpn,k_p}} #1\!\diff t
        }\nolimits}
%
\newcommand{\sumTs}{\mathop{\sum_{{\Ts},k_{\Ts}}}\nolimits}
\newcommand{\sumEs}{\mathop{\sum_{{\Es},k_{\Es}}}\nolimits}
%\newcommand{\unhkTs}{\mathop{
%        \frac{\uSc(\tpn{k_{{\Ts}}})\!+\!\uSc(\tpn{k_{{\Ts}}\!-1})}{2}
%        }\nolimits}
\newcommand{\unhkTs}{\mathop{
        {\CAL{M}^{k_{\Ts}}\!(u_{h,\Dt})}
        }\nolimits}
%\newcommand{\fnhkTs}{\mathop{
%        \frac{\fSc(\tpn{k_{\Ts}})+\fSc(\tpn{k_{\Ts}-1})}{2}
%        }\nolimits}
\newcommand{\fnhkTs}{\mathop{
        {\CAL{M}^{k_{\Ts}}\!(f_{h,\Dt})}
        }\nolimits}



==> Styles/addstyle.tex <==
%
% File di definizioni aggiuntive
%
%
\newcommand{\accapo}{\vspace*{11pt}}
%
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
%\newtheorem{remark}{Remark}
%\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}
\newtheorem{notation}{Notation}
%\newtheorem{evidenzia}{}
\newtheorem{algorithm}{Algorithm}
\newtheorem{assumption}{Assumption}
%
%
%
\newcommand{\qmatrix}[1]{\left[\matrix{#1}\right]}
%
\renewcommand{\ds}{\displaystyle}
\newcommand{\ts}{\textstyle}
\newcommand{\Ds}[1]{{\displaystyle #1}}
%
%
\newcommand{\eng}{\selectlanguage{english}}


==> Styles/common_styles.tex <==
%\usepackage[italian]{babel}
\usepackage[english]{babel}
\usepackage{draftcopy}
\usepackage{enumerate}
\usepackage{latexsym}
\usepackage{amsfonts,amssymb}
\usepackage{rotating}
\usepackage{color}
\usepackage{amsbsy,bm}
\usepackage{graphicx}
\usepackage{ulem}
%
\usepackage{etex}
\usepackage{pictexwd}
%
%
%
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\eps}{{\tt eps}}
%\newcommand{\upm}{\varepsilon_{\mathrm m}}
\newcommand{\upm}{{\tt u}}
\newcommand{\tol}{{\tt tol}}
\newcommand{\ds}{\displaystyle}
\newcommand{\m}{{\tt OCTAVE/MATLAB}}

\newcommand{\newf}{\end{frame}\begin{frame}}
\newcommand{\norma}[1]{\mathop{\left\|\,#1\,\right\|}\nolimits}
\newcommand{\ist}[1]{{\tt >> #1}}
%
\newcommand{\F}{\mathbb{F}(\beta,t,L,U)}   % Insieme di numeri macchina
\newcommand{\fl}{{\rm fl}}   % approssimazione a numeri macchina
\newcommand{\ffl}[1]{{\rm fl}(#1)}   % approssimazione a numeri macchina

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{property}{Property}
\newtheorem{proposition}{Proposition}
\newtheorem{exercise}{Esercise}
\newtheorem{evidenzia}{}


==> Styles/prima_pagina.tex <==
\author{Alessandro D'Auria}
\institute{
\begin{columns}[t,onlytextwidth]
\column{.2\textwidth}

\includegraphics[scale=0.17]{../Immagini/logo}
\column{.8\textwidth}
GEOSCORE Group\\
Dipartimento di Scienze Matematiche ''Giuseppe Luigi Lagrange``\\
Politecnico di Torino\\
{\tt alessandro.dauria@polito.it}\\
\vskip15pt
{\tiny Joint work with}: S. Berrone, A. Borio.
\end{columns}
\includegraphics[width=0.5\linewidth]{./logo_eccellenza.jpg}
}
%
\date{
\vskip6pt
\begin{small}{MAFELAP 2019}\end{small} - \begin{footnotesize}{Jun 20, London}\end{footnotesize}\\
}

\logo{\includegraphics[height=0.5cm]{../Immagini/marchio}}


==> Styles/sandra.symbols.tex <==
\newcommand{\dg}{\, \mathrm{d}\gamma}
\newcommand{\phiik}{\phi_{i,k}}
\newcommand{\phijk}{\phi_{j,k}}
\newcommand{\phiil}{\phi_{i,\ell}}
\newcommand{\phijl}{\phi_{j,\ell}}
\newcommand{\psiik}{\psi_{i,k}^S}
\newcommand{\psijk}{\psi_{j,k}^S}
\newcommand{\psiil}{\psi_{i,\ell}^S}
\newcommand{\psijl}{\psi_{j,\ell}^S}
\newcommand{\psimkm}{\psi_{m,k}^-}
\newcommand{\psimkp}{\psi_{m,k}^+}
\newcommand{\psimlm}{\psi_{m,\ell}^-}
\newcommand{\psimlp}{\psi_{m,\ell}^+}
\newcommand{\TENS}[1]{\mathop{\mathbf{#1}}\nolimits}
\newcommand{\hik}{h_{i,k}}
\newcommand{\hjk}{h_{j,k}}
\newcommand{\hil}{h_{i,\ell}}
\newcommand{\hjl}{h_{j,\ell}}
\newcommand{\uik}{u_{i,k}^S}
\newcommand{\ujk}{u_{j,k}^S}
\newcommand{\uil}{u_{i,\ell}^S}
\newcommand{\ujl}{u_{j,\ell}^S}
\newcommand{\umkm}{u_{m,k}^-}
\newcommand{\umkp}{u_{m,k}^+}
\newcommand{\umlm}{u_{m,\ell}^-}
\newcommand{\umlp}{u_{m,\ell}^+}

\newcommand{\card}{\mathrm{card}}

\newcommand{\Si}{\CAL{S}_i}

\newcommand{\fracset}{\mathfrak{I}}
\newcommand{\traceset}{\mathfrak{M}}

\newcommand{\rosso}[1]{{\color{red}#1}}
\newcommand{\blu}[1]{\begin{color}{blue}#1\end{color}}
\newcommand{\verde}[1]{\begin{color}{green}#1\end{color}}

\newcommand{\mockalph}[1]{}
\newcommand{\precision}[1]{\pgfmathprintnumber[fixed,fixed zerofill,precision=1]{#1}}
\newcommand{\myround}[1]{\pgfmathprintnumber[fixed,fixed zerofill,precision=2]{#1}}

